Leveling Up Together: Fostering Positive Growth and Safe Online Spaces for Teen Roblox Developers

Creating games together is both a playful and effective way to develop skills in computational thinking, collaboration, and more. However, game development can be challenging for younger developers who lack formal training. While teenage developers frequently turn to online communities for peer support, their experiences may vary. To better understand the benefits and challenges teens face within online developer communities, we conducted interviews with 18 teenagers who created games or elements in Roblox and received peer support from one or more online Roblox developer communities. Our findings show that developer communities provide teens with valuable resources for technical, social, and career growth. However, teenagers also struggle with inter-user conflicts and a lack of community structure, leading to difficulties in handling complex issues that may arise, such as financial scams. Based on these insights, we propose takeaways for creating positive and safe online spaces for teenage game creators.

==> tables/demographics.tex <==
\begin{table}[]
\centering

\begin{tabular}{|c|cccc|}
\hline
\rowcolor[HTML]{E4E4E4} 
\textbf{{Alias}} & \cellcolor[HTML]{E4E4E4}\textbf{\begin{tabular}[c]{@{}c@{}}Age (Gender)\\ m=16.3\end{tabular}} & \textbf{Nationality} & \textbf{Profession}                                                                         & \textbf{\begin{tabular}[c]{@{}c@{}}Roblox Creation\\ Experience\end{tabular}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
C1                                                                 & 18 (M)                                                                                         & South Korea          & 3d Modeling                                                                                 & 7 years                                                                       \\
\rowcolor[HTML]{FFFFFF} 
C2                                                                 & 17 (M)                                                                                         & South Korea          & 3d Modeling                                                                                 & 5 years                                                                       \\
\rowcolor[HTML]{FFFFFF} 
C3                                                                 & 15 (M)                                                                                         & USA                  & Building, Scripting                                                                         & 2 $\sim$3 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C4                                                                 & 16 (M)                                                                                         & South Korea          & Building                                                                                    & 3+ years                                                                      \\
\rowcolor[HTML]{FFFFFF} 
C5                                                                 & 16 (M)                                                                                         & South Korea          & All rounded                                                                                 & \textless 6 months                                                            \\
\rowcolor[HTML]{FFFFFF} 
C6                                                                 & 17 (M)                                                                                         & South Korea          & All rounded                                                                                 & 2 $\sim$3 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C7                                                                 & 18 (M)                                                                                         & South Korea          & Scripting, Modeling, UI, Design                                                             & 2 $\sim$3 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C8                                                                 & 14 (M)                                                                                         & USA                  & Scripting                                                                                   & 2 $\sim$3 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C9                                                                 & 16 (M)                                                                                         & South Korea          & Scripting                                                                                   & \textgreater 3 years                                                          \\
\rowcolor[HTML]{FFFFFF} 
C10                                                                & 15 (M)                                                                                         & South Korea          & Scripting                                                                                   & \textgreater 3 years                                                          \\
\rowcolor[HTML]{FFFFFF} 
C11                                                                & 17 (M)                                                                                         & USA                  & Scripting, 3d Modeling                                                                      & 6 years                                                                       \\
\rowcolor[HTML]{FFFFFF} 
C12                                                                & 16 (M)                                                                                         & Malaysia             & Scripting                                                                                   & 1 $\sim$2 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C13                                                                & 19 (F)                                                                                         & South Korea          & 3d Modeling, UGC                                                                            & 5 years                                                                       \\
\rowcolor[HTML]{FFFFFF} 
C14                                                                & 16 (M)                                                                                         & Spain                & Scripting, 3d Modeling                                                                      & 1 $\sim$2 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C15                                                                & 16 (F)                                                                                         & South Korea          & 3d Modeling, Building                                                                       & 2 $\sim$3 years                                                               \\
\rowcolor[HTML]{FFFFFF} 
C16                                                                & 15 (M)                                                                                         & Japan                & Scripting, GFX, Game designing                                                              & \textgreater 3 years                                                          \\
\rowcolor[HTML]{FFFFFF} 
C17                                                                & 16 (M)                                                                                         & Denmark              & Scripting                                                                                   & \textgreater 3 years                                                          \\
\rowcolor[HTML]{FFFFFF} 
C18                                                                & 15 (M)                                                                                         & South Korea          & \begin{tabular}[c]{@{}c@{}}Scripting, 3d Modeling, \\ Building, GFX, Animation\end{tabular} & 1 $\sim$2 years                                                               \\ \hline
\end{tabular}
\caption{Overview of participants. The profession within Roblox game development had six options (scripting, 3d modeling, building, GFX, animation, game design). }
\label{tab:demographics}
\end{table}

==> tex/00_abstract.tex <==
Creating games together is both a playful and effective way to develop skills in computational thinking, collaboration, and more. However, game development can be challenging for younger developers who lack formal training. While teenage developers frequently turn to online communities for peer support, their experiences may vary. To better understand the benefits and challenges teens face within online developer communities, we conducted interviews with 18 teenagers who created games or elements in Roblox and received peer support from one or more online Roblox developer communities. Our findings show that developer communities provide teens with valuable resources for technical, social, and career growth. However, teenagers also struggle with inter-user conflicts and a lack of community structure, leading to difficulties in handling complex issues that may arise, such as financial scams. Based on these insights, we propose takeaways for creating positive and safe online spaces for teenage game creators. 
